SyncSpecCNN: Synchronized Spectral CNN for 3D Shape Segmentation

In this paper, we study the problem of semantic annotation on 3D models that are represented as shape graphs. A functional view is taken to represent localized information on graphs, so that annotations such as part segment or keypoint are nothing but 0-1 indicator vertex functions. Compared with images that are 2D grids, shape graphs are irregular and non-isomorphic data structures. To enable the prediction of vertex functions on them by convolutional neural networks, we resort to spectral CNN method that enables weight sharing by parameterizing kernels in the spectral domain spanned by graph laplacian eigenbases. Under this setting, our network, named SyncSpecCNN, strive to overcome two key challenges: how to share coefficients and conduct multi-scale analysis in different parts of the graph for a single shape, and how to share information across related but different shapes that may be represented by very different graphs. Towards these goals, we introduce a spectral parameterization of dilated convolutional kernels and a spectral transformer network. Experimentally we tested our SyncSpecCNN on various tasks, including 3D shape part segmentation and 3D keypoint prediction. State-of-the-art performance has been achieved on all benchmark datasets.

==> tex/diagnosis.tex <==
\label{sec:diagnosis}


==> tex/old.tex <==
According to \cite{ovsjanikov2012functional}, functional map could be used to align spectral domain of different shapes but some rough correspondence among shapes in the spatial domain is needed for its computation. Therefore, a friendly input representation for SpecTN should be able to encode rough spatial correspondences. In addition, since functional map is used to synchronize different spectral domains, we need to provide knowledge about these spectral domains to SpecTN. To feed a representation encoding rough correspondences to SpecTN, we first use the hierarchical joint alignment algorithm described in \cite{shapenet2015} to align all the input shapes into a canonical 3D space, where rough correspondences among different shapes could be obtained by simple nearest neighbor search. Then we voxelize input shapes and use voxel cells to indicate correspondence among different shapes, namely two vertices are in correspondence if they fall into the same voxel cell. In this way, we could get rid of cumbersome pairwise correspondences computation. This voxelized representation of jointly aligned input shapes provides rough correspondences, thus very friendy for functional map prediction. To add knowledge about different spectral domains in the input, we convert eigenbases $\myvec{B}=\{\myvec{b_i}\}$ of each $\graph$, which are represented as vertex functions, into voxel functions $\myvec{B_v}=\{\myvec{b_{vi}}\}$. And the shape voxel representation together with voxel functions $\myvec{B_v}$ will serve as the input to SpecTN.

Converting graph vertex function into voxel function is pretty straightforward in our setting and we simply need to transport the vertex function value to corresponding voxel cells where the vertex lies in. If multiple vertex function values are transported into a same voxel cell, average pooling will be done to get the voxel function value. If no vertex function value is transported into a voxel cell, $\myvec{0}$ will be assigned to it.


The second challenge in our design is about optimizing SpecTN. High dimensional spectral transformation estimation is harder in nature compared with low dimensional spatial transformation. To facilitate learning, we adopt two approaches: using a good initialization and adding regularizations. To be specific, we pre-train the SpecTN in a supervised fashion so that it predicts functional map to roughly canonicalize different spectral domains, then we fine-tune SpecTN while training the whole SyncSpecCNN with an end task such as shape segmentation. Regularizations are used during training to force the output $C$ of SpecTN to be close to an orthogonal map, namely we add $||CC^T-I||_F^2$ into the overall loss function. The pre-training step is crucial since it provides a good initialization for fine-tuning. To obtain rough functional map for pre-training, we first construct an average shape graph $\bar{\graph}_v$ in the voxelized 3D space where we have jointly aligned the input shapes. Then we estimate functional maps to align each individual spectral domain, approximated by $\myvec{B_v}$, with the average spectral domain, depicted by $\bar{\myvec{B}}_v$. Here $\bar{\myvec{B}}_v$ denotes the eigenbases corresponding to the graph Laplacian of $\bar{\graph}_v$. The average shape graph $\bar{\graph}_v$ lies in the voxelized 3D space, with a vertex set $\vertex_v$ including all the voxel cells and an edge set $\edge_v$ describing connections among voxel cells. $\bar{\graph}_v$ is obtained by simply associating every vertex in each $\graph$ with some voxel cell and adding every edge weight in each $\graph$ onto some connection weight between voxels. \todo{show visualization for laplacian eigenvectors of the average graph}. We use voxel functions $\myvec{B_v}$ instead of $\myvec{B}$ to approximate the spectral domain of each individual $\graph$ since they are defined on the same voxelized 3D space as $\bar{\myvec{B}}_v$ and the functional map $C_v$ aligning $\myvec{B_v}$ with $\bar{\myvec{B}}_v$ could be computed through simple matrix multiplication $C_v=\bar{\myvec{B}}_v^T\bar{\myvec{B}}_v$. The computed functional map will serve as supervision and SpecTN is pre-trained to minimize the loss function $||C-C_v||_F^2$.

The resolution of the voxelized 3D space does not need to be high since we are only focusing on synchronizing low-frequency end of different spectral domains. We use a small volumetric CNN \cite{qi2016volumetric} for our SpecTN and there is an regression layer in the end of SpecTN to predict the functional map.
